ConfuciuX: Autonomous Hardware Resource Assignment for DNN Accelerators using Reinforcement Learning

DNN accelerators provide efficiency by leveraging reuse of activations/weights/outputs during the DNN computations to reduce data movement from DRAM to the chip. The reuse is captured by the accelerator's dataflow. While there has been significant prior work in exploring and comparing various dataflows, the strategy for assigning on-chip hardware resources (i.e., compute and memory) given a dataflow that can optimize for performance/energy while meeting platform constraints of area/power for DNN(s) of interest is still relatively unexplored. The design-space of choices for balancing compute and memory explodes combinatorially, as we show in this work (e.g., as large as O(10^(72)) choices for running \mobilenet), making it infeasible to do manual-tuning via exhaustive searches. It is also difficult to come up with a specific heuristic given that different DNNs and layer types exhibit different amounts of reuse. In this paper, we propose an autonomous strategy called ConfuciuX to find optimized HW resource assignments for a given model and dataflow style. ConfuciuX leverages a reinforcement learning method, REINFORCE, to guide the search process, leveraging a detailed HW performance cost model within the training loop to estimate rewards. We also augment the RL approach with a genetic algorithm for further fine-tuning. ConfuciuX demonstrates the highest sample-efficiency for training compared to other techniques such as Bayesian optimization, genetic algorithm, simulated annealing, and other RL methods. It converges to the optimized hardware configuration 4.7 to 24 times faster than alternate techniques.

==> figure/area_breakdown.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/area_breakdown.pdf}
\end{center}
\vspace{-0.40cm}
\caption{\small Area breakdown of the solutions for MobileNet-V2 and ResNet-50 (Obj.(min.):Latency, Cstr:IoT area).}
\vspace{-0.1cm}
\label{fig:area_breakdown}
\end{figure}




==> figure/generalization.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/generalization.pdf}
\end{center}
\vspace{-0.40cm}
\caption{\small The generalizable network.}
\vspace{-0.1cm}
\label{fig:generalization}
\end{figure}




==> figure/highlevel.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/fig1.pdf}
\end{center}
\vspace{-0.40cm}
\caption{\small Design-flow with \system.} 
% \TK{Don't forger to change RAMAN to ConficuiX in all figures}
\vspace{-0.1cm}
\label{fig:highlevel}
\end{figure}


==> figure/maestro_7loop.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/maestro_7loop.png}
\end{center}
\vspace{-0.40cm}
\caption{The 7 loop of CNN.}
\vspace{-0.1cm}
\label{fig:7loop}
\end{figure}


==> figure/policy_network.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/policy_network.png}
\end{center}
\vspace{-0.40cm}
\caption{The policy network.}
\vspace{-0.1cm}
\label{fig:policy_network}
\end{figure}


==> figure/resource_allocation.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/dataflow_fig.pdf}
\end{center}
\vspace{-0.40cm}
\caption{\small HW performance under different resource allocations for the first layer of \mobilenet.}
\vspace{-0.1cm}
\label{fig:dataflow_hw}
\end{figure}


==> sections/07-Discussion.tex <==
\section{Discussions}
\label{sec:discussions}
\subsubsection{Generalization}
Another crucial benefit of RL is the potential to do transfer learning, which means the learned policy on the seen models can be generalized to unseen models. We could decouple backbone of RL agent into encoder and decoder, as shown in \autoref{fig:generalization} Encoder accounts for realizing the entire model shape. Decoder accounts for assigning the resources with the knowledge of the entire model information and the current layer information. With this decoupled structure, the decoder has the potential to be generalized to other unseen network. The benefit of the generalization is the sampling efficiency. Since the RL agent can start from a good initial point with the transferred knowledge. It could lead to optimal points much faster. We leave this extension as our future work.

% \input{figure/generalization}

==> tables/gemm.tex <==



\begin{table}[t]
\centering
\caption{\small \system on GEMM-based models.}
\includegraphics[width=1\linewidth]{Figures/tb5.pdf}
\label{table:gemm}
\end{table}


==> tables/neat_table.tex <==
\begin{table}[]
\caption{The major functions in NEAT.}
\vspace{-0.3cm}
\begin{tabular}{|
>{\columncolor[HTML]{C0C0C0}}l |
>{\columncolor[HTML]{EFEFEF}}r |l|}
\hline
\multicolumn{2}{|r|}{\cellcolor[HTML]{EFEFEF}evaluate}                                                                                    & \begin{tabular}[l]{@{}l@{}}Inference the NN and compute its fitness value.\end{tabular} \\ \hline
\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} }                                                                                & createNet    & \begin{tabular}[l]{@{}l@{}} Decode the genes to nodes and connections, solve\\the dependency among nodes, and formulate them\\ into NN topology.\end{tabular} \\ \cline{2-3} 
\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} }                                                                                & mutate  & Tweak an parent's gene to reproduce individuals. \\ \cline{2-3} 
\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} }                                                                                & crossover & Mixture two parents' gene to reproduce individuals. \\ \cline{2-3} 
\multirow{-4}{*}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}ev-\\ ol-\\ ve\end{tabular}}} & speciate & \begin{tabular}[l]{@{}l@{}} Classify individual by their topology similarity so that \\they only compete within group. It protects the young\\ individuals from elimination before well-evolved. \end{tabular}\\ \hline
\end{tabular}
\vspace{-0.1cm}
\label{table:neat}
\end{table}

%searching of similar topologies and distance comparing\




==> tables/resource_utilize.tex <==
\begin{table}[]
\caption{Resource utilization.}
\vspace{-0.3cm}
\begin{tabular}{|l|l|l|}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}DSP}  & LUT & FF \\ \hline
                                                      &     &    \\ \hline
\end{tabular}
\vspace{-0.1cm}
\label{table:resource}
\end{table}

==> tables/tb_dataflow.tex <==


\begin{table}[t]
\centering
\caption{\small \system on other dataflow style.}
\includegraphics[width=1\linewidth]{Figures/tb4.pdf}
\label{table:compare_dataflow}
\end{table}

